PQk-means: Billion-scale Clustering for Product-quantized Codes

Data clustering is a fundamental operation in data analysis. For handling large-scale data, the standard k-means clustering method is not only slow, but also memory-inefficient. We propose an efficient clustering method for billion-scale feature vectors, called PQk-means. By first compressing input vectors into short product-quantized (PQ) codes, PQk-means achieves fast and memory-efficient clustering, even for high-dimensional vectors. Similar to k-means, PQk-means repeats the assignment and update steps, both of which can be performed in the PQ-code domain. Experimental results show that even short-length (32 bit) PQ-codes can produce competitive results compared with k-means. This result is of practical importance for clustering in memory-restricted environments. Using the proposed PQk-means scheme, the clustering of one billion 128D SIFT features with K = 10^5 is achieved within 14 hours, using just 32 GB of memory consumption on a single computer.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	mm17.tex


PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF} compress


compress_eachimg:
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=img/k_time/output.pdf img/k_time/k_time.pdf
#	rm img/k_time/k_time.pdf
#	mv img/k_time/output.pdf img/k_time/k_time.pdf
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=img/large_exp_yfcc100m/output.pdf img/large_exp_yfcc100m/yfcc100m_k_error.pdf
#	rm img/large_exp_yfcc100m/yfcc100m_k_error.pdf
#	mv img/large_exp_yfcc100m/output.pdf img/large_exp_yfcc100m/yfcc100m_k_error.pdf
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=img/large_exp_yfcc100m/output.pdf img/large_exp_yfcc100m/yfcc100m_k_time.pdf
#	rm img/large_exp_yfcc100m/yfcc100m_k_time.pdf
#	mv img/large_exp_yfcc100m/output.pdf img/large_exp_yfcc100m/yfcc100m_k_time.pdf
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=img/memory_error/output.pdf img/memory_error/memory_error.pdf
#	rm img/memory_error/memory_error.pdf
#	mv img/memory_error/output.pdf img/memory_error/memory_error.pdf
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=img/n_error/output.pdf img/n_error/n_error.pdf
#	rm img/n_error/n_error.pdf
#	mv img/n_error/output.pdf img/n_error/n_error.pdf
#	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=img/n_time/output.pdf img/n_time/n_time.pdf
#	rm img/n_time/n_time.pdf
#	mv img/n_time/output.pdf img/n_time/n_time.pdf


# Added by Y. Matsui
compress: mm17.pdf
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=output.pdf mm17.pdf
	#gs -o output.pdf -dNoOutputFonts -sDEVICE=pdfwrite mm17.pdf  # Converts all texts to vector lines
	rm mm17.pdf
	mv output.pdf mm17.pdf





%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

